Agent-based Model of Initial Token Allocations: Evaluating Wealth Concentration in Fair Launches

With advancements in distributed ledger technologies and smart contracts, tokenized voting rights gained prominence within Decentralized Finance (DeFi). Voting rights tokens (aka. governance tokens) are fungible tokens that grant individual holders the right to vote upon the fate of a project. The motivation behind these tokens is to achieve decentral control. Because the initial allocations of these tokens is often un-democratic, the DeFi project Yearn Finance experimented with a fair launch allocation where no tokens are pre-mined and all participants have an equal opportunity to receive them. Regardless, research on voting rights tokens highlights the formation of oligarchies over time. The hypothesis is that the tokens' tradability is the cause of concentration. To examine this proposition, this paper uses an Agent-based Model to simulate and analyze the concentration of voting rights tokens post fair launch under different trading modalities. It serves to examine three distinct token allocation scenarios considered as fair. The results show that regardless of the allocation, concentration persistently occurs. It confirms the hypothesis that the disease is endogenous: the cause of concentration is the tokens tradablility. The findings inform theoretical understandings and practical implications for on-chain governance mediated by tokens.

==> sections/07_outlook.tex <==
\subsection{Outlook}
The topic of voting rights tokens and initial token allocations provides noteworthy research streams. At once, theorists in \ac{IS} investigated token design as part of wider blockchain (eco-)systems and economies, not least \citet{oliveira2018token}, \citet{hulsemann_walk_2019}, and \citet{drasch2020token}. Ample literature dedicated to blockchain governance and more particularly \textit{on-chain} governance, collectively provides a sound foundation for future research. We foresee two principle streams for investigation.

At once, the study of voting rights tokens in \textit{non-custodial} (the tokens are unregistered) spaces. Voting rights tokens, given their speculative nature as assets and lack of actual use for voting, are here 'usage-based' only in a "subordinate sense" \citep[21]{barbereau_decentralised_2022}. Research here, may at once consider the application of voting rights tokens within individual \ac{DeFi} projects. Exemplary here is the case study by \citet{brennecke2022central} on MakerDAO and the voting rights token MKR. Alternatively, theorists can turn towards law and build on the work of \citet{zetzsche_decentralized_2020} to discuss efficiencies and failures of \textit{embedded regulation}.

The second stream, then, may consider the embedding of voting rights in tokens within \textit{custodial} (the tokens are registered as securities) spaces. Few have, however, dedicated attention to the \textit{actual} utility and use of voting rights tokens within corporate governance processes. The exception, to our knowledge, is the primer by \citet{yermack2017corporate} on \ac{DLT}-based corporate governance in general, as well as subsequent work by \citet{lambert2021security} on attaching voting rights to security tokens in the context of capital raising specifically. The authors consider the role of security tokens with embedded voting rights as part of a study on factors associated with successful capital raising. 

At the intersection between these streams are works that consciously seek to improve the governance processes and, for instance, avoid a specific problematic such as concentration of power. Notable here is the work of \citet{tsoukalas2020token} which considers the effectiveness of a weighting system for tokenized voting in a decentralized system. 

